The Multiobjective Optimization of a Prismatic Drive

The multiobjective optimization of Slide-o-Cam is reported in this paper. Slide-o-Cam is a cam mechanism with multiple rollers mounted on a common translating follower. This transmission provides pure-rolling motion, thereby reducing the friction of rack-and-pinions and linear drives. A Pareto frontier is obtained by means of multiobjective optimization. This optimization is based on three objective functions: (i) the pressure angle, which is a suitable performance index for the transmission because it determines the amount of force transmitted to the load vs. that transmitted to the machine frame; (ii) the Hertz pressure used to evaluate the stresses produced on the contact surface between cam and roller; and (iii) the size of the mechanism, characterized by the number of cams and their width.

==> 05Summary.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{SUMMARY OF RESULTS AND CONCLUSIONS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This paper dealt with the optimization of Slide-o-Cam mechanism
based on the Pressure angle and Hertz pressure. The kinematic
constraints of the Orhtoglide was used to defined to pitch and the
input torque but the result was general. For a given input torque
and pitch, the optimal design parameters of the cam, i.e.
$\phi_{cam}$ and $\phi_{bear}$ are computed when we consider the
maximal admissible pressure angle $\mu_{max}$ as a constraint and
the strength of the material.

Conversely to previous works, the optimization of the cam parameters
based on the Hertz pressure does not converge toward the results
obtained by an optimization based on the pressure angle. The optimal
values are not the ones obtained for a minimum radius of the roller
$a_4$ and a minimum diameter of the cam $\phi_{cam}$. Further
research on the fatigue of the cam and the bearing are currently
carried on.


==> 06Acknowledgments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ACKNOWLEDGMENTS}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
This research work was partly made by \'Emilie Bouyer during her
internship at McGill University from April, the 15th to August, the
31st 2006.

